Adaptive Total Variation Stable Local Timestepping for Conservation Laws

This paper proposes a first-order total variation diminishing (TVD) treatment for coarsening and refining of local timestep size in response to dynamic local variations in wave speeds for nonlinear conservation laws. The algorithm is accompanied with a proof of formal correctness showing that given a sufficiently small minimum timestep the algorithm will produce TVD solution for nonlinear scalar conservation laws. A key feature of the algorithm is its formulation as a discrete event simulation, which allows for easy and efficient parallelization using existing software. Numerical results demonstrate the stability and adaptivity of the method for the shallow water equations. We also introduce a performance model to load balance and explain the observed performance gains. Performance results are presented for a single node on Stampede2's Skylake partition using an optimistic parallel discrete event simulator. Results show the proposed algorithm recovering 59%-77% of the theoretically achievable speed-up with the discrepancies being attributed to the cost of computing the CFL condition and load imbalance.

==> images/config.tex <==
%This is a file of macros which tracks numbers used throughout the paper
%Do not edit this file. Rather change images/generate_performance_results.py

\begin{tabular}{|c|c|c|c|c|c|c|}\hline
Initial Condition & warp\_type & Runtime & n\_elments & n\_actors & t\_end & lambda\_by\_dx\_max\\\cline{1-7}
\multirow{4}{*}{lake\_at\_rest} & \multirow{2}{*}{uniform} & mpi & 500000 & 48 & 1.0 & 252500 \\\cline{3-7}
& & deva & 500000 & 288 & 1.0 & 505000 \\\cline{2-7}
& \multirow{2}{*}{polynomial} & mpi & 500000 & 48 & 0.2 & 4460833.332 \\\cline{3-7}
& & deva & 500000 & 288 & 0.2 & 8921666.665 \\\cline{1-7}
\multirow{4}{*}{carrier\_greenspan} & \multirow{2}{*}{uniform} & mpi & 500000 & 48 & $2\pi$ & 266512.5758 \\\cline{3-7}
& & deva & 500000 & 288 & $2\pi$ & 533025.1515 \\\cline{2-7}
& \multirow{2}{*}{polynomial} & mpi & 500000 & 48 & $2\pi$ & 2875945.721 \\\cline{3-7}
& & deva & 500000 & 288 & $2\pi$ & 5751891.441 \\\cline{1-7}
\end{tabular}

==> sections/artifact.tex <==
% LaTeX template for Artifact Description appendix used for SC17
% V20170220
%% V20170220
% (C)opyright 2017

% Derived with permission by Michael Heroux (Sandia National Laboratories, St. John's University, MN)
% from ae-20160509.tex 
% written by Grigori Fursin (cTuning foundation, France and dividiti, UK) 
% and Bruce Childers (University of Pittsburgh, USA)
% (C)opyright 2014-2016

\appendix\section{Artifact Description: Adaptive Total Variation Stable Local Timestepping for Conservation Laws}
\label{sec:artifact}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Abstract}

As part of the Association for Computing Machinery's reproducibility initiative, this artifact outlines the details of generating the performance comparison in ``Adaptive Total Variation Stable Local Timestepping for Conservation Laws''.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Description (artifact meta information)}
{\small
\begin{itemize}
  \item {\bf Algorithm: } Finite Volume Code with Adaptive Local Timestepping
  \item {\bf Program: } python, C++14
  \item {\bf Compilation: } GNU C++14 Compiler
%  \item {\bf Transformations: }
%  \item {\bf Binary: }
%  \item {\bf Data set: }
  \item {\bf Operating System: } CentOS Linux release 7.6.1810
  \item {\bf Run-time environment: } Stampede2/Skylake partition
%  \item {\bf Hardware: }
%  \item {\bf Run-time state: }
  \item {\bf Execution: } Parallel/Shared Memory
%  \item {\bf Output: }
  \item {\bf Experiment workflow: } Compile; Preprocess meshes; Run simulation.
%  \item {\bf Experiment customization: }
  \item {\bf Publicly available?: } Yes
\end{itemize}
}

\subsubsection{How software can be obtained}
Software is not yet open-source.

\subsubsection{Software dependencies}
Specific version numbers  of software are provided in Table \ref{tab:version}.

\begin{table}
{
\footnotesize
\caption{Version numbers and git hashes of dependencies}
\label{tab:version}
\begin{center}
\begin{tabular}{|c| c|}
\hline
Software & Stampede2 \\
\hline
\pkg{gcc} & 7.1.0\\
\hline
MPI implementation&  impi/17.0.3 \\
\hline
Devastator & 2c0e160\\
\hline
Python & 3.7.3\\
\hline
\pkg{Gurobi} & 9.0.0\\
\hline
\end{tabular}
\end{center}
}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Installation}
Assuming all dependencies are available, the code uses GNU Makefile to build both versions of the code. The Devastator version of the code can be generated using
\begin{lstlisting}
    make threads=48 problem=XXX ics=YYY
\end{lstlisting}
where equation type \lstinline{problem} may either be set to \lstinline{burgers} or \lstinline{swe}. For solving Burgers' equation, \lstinline{ics} may be set to one of \lstinline{constant}, \lstinline{shockwave}, or \lstinline{rarefaction}, and for solving the shallow water equations, \lstinline{ics} may be set to one of \lstinline{constant}, \lstinline{dambreak}, or \lstinline{carrier-greenspan}.
For the MPI version, the make target is \lstinline{lts-mini-app.mpi}. The problem type and initial conditions can be set using the same \lstinline{problem} and \lstinline{ics} flags used for the Devastator executable.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Experiment workflow}
\begin{table}
{\footnotesize
\caption{Shallow water equations configuration for MPI-Devastator Performance Comparison}
\label{tab:env-vars-perf-comp}
\centering
\input{images/config}
}
\end{table}

The workflow requires setting environment variables including input (\lstinline{lts_input_dir}) and output (\lstinline{lts_output_dir}) folders and the name of the mesh file (\lstinline{lts_mesh_file}). The parameters for the runs in Section~\ref{sec:performance-results} are shown in Table~\ref{tab:env-vars-perf-comp}.
From the root directory, the work flow then requires generating the mesh and mesh splitters as well as any input files,
\begin{lstlisting}
    python scripts/mesh_generator.py,
\end{lstlisting}
generating an actor partition, which is only needed for the Carrier-Greenspan problem,
\begin{lstlisting}
    python scripts/partition_actors.py,
\end{lstlisting}
and running the executable. For the synchronous MPI version, we use TACC's \lstinline{ibrun} launcher.

Lastly, we remark that for the polynomial meshes using an MPI simulation, we generate the mesh using an appropriately set \lstinline{warp_type} environment variable, but then manually overwrite the splitters file using the splitters associated with a uniform warp type.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Evaluation and expected result}
Each simulation run will return the execution time in microseconds to the standard output, and additional output information is written to the output directory.

